Epistemic Uncertainty Aware Semantic Localization and Mapping for Inference and Belief Space Planning

We investigate the problem of autonomous object classification and semantic SLAM, which in general exhibits a tight coupling between classification, metric SLAM and planning under uncertainty. We contribute a unified framework for inference and belief space planning (BSP) that addresses prominent sources of uncertainty in this context: classification aliasing (classier cannot distinguish between candidate classes from certain viewpoints), classifier epistemic uncertainty (classifier receives data "far" from its training set), and localization uncertainty (camera and object poses are uncertain). Specifically, we develop two methods for maintaining a joint distribution over robot and object poses, and over posterior class probability vector that considers epistemic uncertainty in a Bayesian fashion. The first approach is Multi-Hybrid (MH), where multiple hybrid beliefs over poses and classes are maintained to approximate the joint belief over poses and posterior class probability. The second approach is Joint Lambda Pose (JLP), where the joint belief is maintained directly using a novel JLP factor. Furthermore, we extend both methods to BSP, planning while reasoning about future posterior epistemic uncertainty indirectly, or directly via a novel information-theoretic reward function. Both inference methods utilize a novel viewpoint-dependent classifier uncertainty model that leverages the coupling between poses and classification scores and predicts the epistemic uncertainty from certain viewpoints. In addition, this model is used to generate predicted measurements during planning. To the best of our knowledge, this is the first work that reasons about classifier epistemic uncertainty within semantic SLAM and BSP.

==> 03-Approach-Concept-2.tex <==
%
TBD

==> 03-Approach-Concept.tex <==
%
We propose an approach for active SLAM that takes into account epistemic classifier uncertainty, allowing us to plan for reducing or increasing it, while utilizing the coupling between classifier outputs and relative pose with a classifier uncertainty model. For simplicity, we will present our approach initially for the single object myopic, then expand to a multi object setting, and finally address the more general non-myopic case. For the myopic case, we can write objective function Eq.~\eqref{eq:Obj_Func_Max} as follows:
%
\begin{equation}
\begin{split}
J(b[\lambda_k],a_k) = \int_{z_{k+i}}
\prob{z_{k+i}|\his_k,a_k} \cdot  r(b[\lambda_{k+i}]) dz_{k+i}.
\end{split}
\end{equation}
%
The above equation can be written in a sample form, where the future measurements are directly sampled from $\prob{z_{k+1}|\his_k,a_k}$:
%
\begin{equation}
J(b[\lambda_k],a_{k:k+L}) = \frac{1}{N_z} \sum_{z_{k+1}} r(b[\lambda_{k+1}]),
\end{equation}
%
where $N_z$ is the number of $z_{k+1}$ samples.
The approach considers future belief over posterior class probability, i.e. $b[\lambda_{k+1}]$, which accounts both for posterior classification of an object via the expectation, and the posterior model uncertainty via its spread. The $b[\lambda_{k+1}]$ representation is more expressive than a single class probability vector representation, and it can reflect four possible archetypes, as seen in Fig.~\ref{fig:simplex_figures}. Fig.~\ref{fig:Fig_Unknown_Unknown} presents a scenario when the parameters of $b[\lambda_k]$ are close to 1; it represents a case where the inputs to the classifier are totally alien, therefore the output is completely unpredictable. Fig.~\ref{fig:Fig_Known_Known} represent a case where the classifier can safely identify the object with high degree of certainty, i.e. the input is close to the training set. Intuitively, this is the case that we aim for, and generally has the highest reward. Fig.~\ref{fig:Fig_Known_Unknown} represents a case where the classifier certainly can't disambiguate between different classes, i.e. the classifier "knows" that it doesn't know. This can be resulted from ambiguity in the training set between different classes, when objects from different classes look identical from certain viewpoints. Finally, Fig.~\ref{fig:Fig_Uncertain_Edge} represent a case where the classifier can vaguely infer the object class, but it's still far from the training set (e.g. a car of an unusual shape that there are no similar images in the training set), therefore with a large degree of uncertainty.

The belief $b[\lambda_{k+1}]$, as defined by Eq.~\eqref{eq:Belief_Lambda_Def}, is conditioned both on geometric $z^g_{1:k+1}$ and semantic measurements as a $\{ \loggamma_{1:k+1} \}$ cloud. In our approach, we represent $b[\lambda_{k+1}]$ by a set of $\lambda_{k+1}$ particles; Each particle is a class probability vector $\prob{c|z^g_{1:k+1},\loggamma_{1:k+1}(w)}$ that is conditioned on the same $z^g_{1:k+1}$ for all particles, and a \emph{sequence} $\loggamma_{1:k+1}(w)$ given predetermined classifier weight, essentially giving every particle its own classifier. Each $w$ is constant throughout the scenario with the reasoning of keeping the number of particles constant throughout the scenario, thus avoiding to manage an exponentially increasing number of components (such as in \cite{Tchuiev18ral}). This can be achieved by, for example,  training multiple models on the same dataset via bootstrapping, or re-using classifier weight sets created by MC-dropout.

General BSP approaches require generating predicted measurements, and using those, infer the future state and compute the appropriate reward. In the following sections, we will tackle those two problems, thus detailing our BSP approach.



%The $b[\lambda_{k+1}]$ representation is more expressive than a single class probability vector representation, and it can reflect four possible archtypes, as seen in Fig.~\ref{fig:simplex_figures}. Fig.~\ref{fig:Fig_Unknown_Unknown} presents a scenario when the parameters of $b[\lambda_k]$ are close to 1; it represents a case where the inputs to the classifier are totally alien, therefore the output is completely unpredictable. Fig.~\ref{fig:Fig_Known_Known} represent a case where the classifier can safely identify the object with high degree of certainty, i.e. the input is close to the training set. Intuitively, this is the case that we aim for, and generally has the highest reward. Fig.~\ref{fig:Fig_Known_Unknown} represents a case where the classifier certainly can't disambiguate between different classes, i.e. the classifier "knows" that it doesn't know. This can be resulted from ambiguity in the training set between different classes, when objects from different classes look identical from certain viewpoints. Finally, Fig.~\ref{fig:Fig_Uncertain_Edge} represent a case where the classifier can vaguely infer the object class, but it's still far from the training set (e.g. a car of an unusual shape that there are no similar images in the training set), therefore with a large degree of uncertainty.
%
\begin{figure*}[!htbp]
	
	\begin{subfigure}[b]{0.23\textwidth}
		\includegraphics[width=\textwidth]{Fig_Unknown_Unknown.eps}
		\caption{Unknown-unknown}\label{fig:Fig_Unknown_Unknown}
	\end{subfigure}
	%
	\begin{subfigure}[b]{0.23\textwidth}
		\includegraphics[width=\textwidth]{Fig_Known_Unknown.eps}
		\caption{Known-unknown}\label{fig:Fig_Known_Unknown}
	\end{subfigure}
	%
	\begin{subfigure}[b]{0.23\textwidth}
		\includegraphics[width=\textwidth]{Fig_Known_Known.eps}
		\caption{Known-known}\label{fig:Fig_Known_Known}
	\end{subfigure}
	%
	\begin{subfigure}[b]{0.23\textwidth}
		\includegraphics[width=\textwidth]{Fig_Uncertain_Edge.eps}
		\caption{Uncertain classification}\label{fig:Fig_Uncertain_Edge}
	\end{subfigure}
	
	\vspace{-0.2cm}
	\caption{The 4 archetypes of $b[\lambda_k]$, shown in a 3 dimensional Dirichlet simplex example, where blue to yellow correspond to low to high probability respectively. \textbf{(a)} represents an unknown-unknown, where the classifier doesn't identify the object and the epistemic uncertainty is high. In \textbf{(a)} the classifier will recognize the object is indistinguishable from other object types given that viewpoint. In \textbf{(c)} the classifier recognizes that the object of a certain class with certainty. In \textbf{(d)} the classifier gives preference to one of the classes, but with a high degree of uncertainty.}
	\label{fig:simplex_figures}
\end{figure*} 

%--------------------------------------------------------------
\subsection{Measurement Generation}\label{sec:Sample}

In our approach, we must generate both predicted geometric $z^g_{k+1}$ and semantic $\{ \loggamma_{k+1} \}$  measurements. The former is generated from the geometric measurement model, and is straight forward and standard within BSP literature. On the other hand, generating the later is part of our contribution. 

One approach for generating $\{ \loggamma_{k+1} \}$ is to generate a predicted image $\tilde{I}_{k+1}$, and running the classifier with every weight set on it to get $\{ \loggamma_{k+1} \}$, such that:
%
\begin{equation}
	\gamma_{k+1}(w) = \prob{c|\tilde{I}_{k+1},w,D} \;\; \forall w \in W,
\end{equation}
%
and then transforming every $\gamma_{k+1}$ to $\loggamma_{k+1}$ using Eq.~\eqref{eq:Logit_transformation}. This is a high dimensional problem that requires training a model that must be extremely large to generalize well. An example for this kind of model can be seen in \VT{[CITE]}. 

On the other hand, the approach that we propose generates the measurements via a learned classifier uncertainty model. While a model must be learned for each candidate class, this approach allows us to perform planning over a larger variation of scenarios and thus generalizes better with requiring a large model. We use the LG model presented in Eq.~\eqref{eq:Logistical_Gaussian_PDF} for $\gamma_{k+1}$ sampling. 

As both the geometric and classifier models require relative pose $x^{rel}_{k+1} \doteq x^o \ominus x_{k+1}$ between object and robot, in addition to the object class hypothesis $c$, we must sample $x^{rel}$ and $c$. However the posterior class probability $\lambda_{k+1}$ is conditioned on $w$, thus we have a sampling hierarchy that can be described by the following marginalization scheme:
%
\begin{equation}\label{eq:Future_Likelihood}
\begin{array}{c}
	\prob{z_{k+1}|\his_k,a_k} \approx \\ \frac{1}{|W|} \cdot \sum_w \sum_c \int_{x^{rel}_{k+1}} \likelihoods_{k+1} \cdot b^{c}_w[x^{rel-}_{k+1}] \cdot \lambda_k^c(w) dx^{rel}_{k+1}.
\end{array}
\end{equation}
%
Consider $b^c_w[\poses_k] \doteq \prob{\poses_k|c,w,\his_k}$ as the conditional continuous belief at time $k$ given class hypothesis $c$ and classifier weight $k$, $b^{c}_w[x^{rel-}_{k+1}]$ is the propagated continuous belief constructed directly from $b^c_w[\poses_k]$ by propagating the belief using the motion model $\mathcal{M}_{k+1}$ and marginalizing out the previous poses $x_{0:k}$:
%
\begin{equation}\label{eq:Prop_Belief_Comp}
b^{c}_w[x^{rel-}_{k+1}] = \int_{x_{0:k}} \mathcal{M}_{k+1} \cdot b^{c}_w[\poses_k] dx_{0:k}.
\end{equation}  
%
The marginalization scheme in Eq.~\eqref{eq:Future_Likelihood} induces a generative model:
%
\begin{equation}\label{eq:Sample_Generative_Model}
	\begin{array}{c}
	\{ \loggamma_{k+1} \} \sim \prob{\loggamma_{k+1} | c,x^{rel}_{k+1}} \\
	z^G_{k+1} \sim \prob{z^G_{k+1}|x^{rel}_{k+1}} \\
	x^{rel}_{k+1} \sim \prob{\poses_k|c,w,I_{1:k},\his^g_k,a_k} \cdot \motionmodel_{k+1} \\
	c \sim Cat(\lambda_k(w))\\
	w \sim \prob{w|D}.
	\end{array}
\end{equation}
%
Next, we propose a practical scheme to sample measurements from the above model; For $x^{rel}_{k+1}$ we can take the maximum likelihood estimation given $c$ and $w$, but for $c$ we categorically sample with probabilities $\lambda_k(w)$. If we take the maximum likelihood estimation of $c$, i.e. the largest value  $\lambda_k(w)$, this induces a bias towards the highest probability class realization at time $k$, so the predicted future measurements may only account for the most likely class realization even if the advantage in $\lambda^c_k(w)$ is small. Next, as weight realization $w$ is not weighted, and because we have $|W|$ particles, we sample $c$ and $x^{rel}$ for every $|W|$. Finally, we perform maximum likelihood estimation for $z^g_{k+1}$, and sample $|W|$ times $\loggamma_{k+1}$, creating overall $|W|$ samples of $z^g_{k+1}$, and $|W|^2$ samples of $\loggamma_{k+1}$, i.e. $|W|$ samples of $\{ \loggamma_{k+1} \}$. This sampling scheme is summarized in Alg.~\ref{alg:SamplingStrategy}, with $hb_w[\poses^-_{k+1},c]$ being a hybrid belief that will be detailed in the next section.

\begin{algorithm}[t]
	\caption{Maximum Likelihood Sampling Strategy} 
	\label{alg:SamplingStrategy} 
	\flushleft
	
	\begin{algorithmic}[1]
		
		\Require{Propagated hybrid belief $hb_w[\poses^-_{k+1},c]$.}
		\State{$c \gets \text{Sample}\left(Cat(\lambda_{k})\right)$}
		\State{$x_{k+1},x^o \gets \text{MaximumLikelihood}(b^c_w[\poses^-_{k+1}])$}
		\State{$z^g_k \gets \text{MaximumLikelihood}(\prob{z^g_{k+1}|x_{k+1},x^o})$}
		
		\State{$\{ \loggamma_{k+1} \} \gets \emptyset$}
		\For{$|W|$ times}
		\State{$\{ \loggamma_{k+1} \} \gets $} \par \hskip\algorithmicindent {$ \{ \loggamma_{k+1} \} \cup 
			\text{Sample}(\prob{\loggamma_{k+1}|c,x^o,x_{k+1}})$}
		\EndFor \\
		\Return{$z^g_k,\{ \loggamma_{k+1} \}$}
		
	\end{algorithmic}
\end{algorithm}

%-----------------------------------
\subsection{Inference of Future Belief}\label{sec:MH_single_lambda_inf}

In this section we address the inference of $b[\lambda_{k+1}]$ given geometric measurement $z^g_k$, and semantic cloud measurement $\{ \loggamma_{k+1} \}$, either generated from sampling in Sec.~\ref{sec:Sample} or from raw measurements after the robot took action $a_k$. 

Each class probability $\lambda_{k+1}^c(w)$ within the particle $\lambda_{k+1}(w)$ is updated using the Bayes rule as follows:
%
\begin{equation}
	\lambda_{k+1}^c(w) = \eta \cdot \lambda_{k}^c(w) \cdot \prob{z^g_k,\loggamma_{k+1}(w)|c},
\end{equation}
%
with $\eta$ being a normalizing constant that doesn't affect inference. As our classifier model is viewpoint dependent, we must marginalize $\prob{z^g_k,\loggamma_{k+1}(w)|c}$ over $x^{rel}_{k+1}$ to fully utilize our models as follows:
%
\begin{equation}
	\lambda_{k+1}^c(w) \propto \lambda_{k}^c(w) \int_{x^{rel}_{k+1}} \likelihoods_{k+1} \cdot \motionmodel_{k+1} \cdot b^{c}_w[x^{rel-}_{k+1}] dx^{rel}_{k+1},
\end{equation} 
%
where $b^{c}_w[x^{rel-}_{k+1}]$ is constructed the same as Eq.~\eqref{eq:Prop_Belief_Comp}. Together $b^c_w[\poses_x]$ and $\lambda^c_k(w)$ construct a hybrid belief $hb_w[\poses_k,c]$ as follows:
%
\begin{equation}
	\underbrace{\prob{\poses_k, c | \loggamma_{1:k},\his^g_k}}_{hb_w[\poses_k,c]} = 
	\underbrace{\prob{\poses_k | c, \loggamma_{1:k},\his^g_k}}_{b^c_w[\poses_k]}
	\underbrace{\prob{c | \loggamma_{1:k},\his^g_k}}_{\lambda^c_k(w)},
\end{equation}
%
with $b^c_w[\poses_k]$ as the conditional continuous belief and $\lambda^c_k(w)$ is the discrete attached belief. While we only explicitly consider $\lambda^c_k(w)$ within the inference of $\lambda_{k+1}$, it is dependent on $b^c_w[\poses_k]$ as well, taking the viewpoint dependency into account. $b^c_w[\poses_k]$ is incrementally updated as well using the standard SLAM formulation presented in literature:
%
\begin{equation}\label{eq:Hybrid_Cont}
b^c_{w}[\poses_{k+1}] \propto b^c_w[\poses_{k}] \cdot \motionmodel_{k+1} \cdot \likelihoods_{k+1}.
\end{equation}
%
Practically, for every $w \in W$, we maintain $b^c_w[\poses_k]$ with the accompanying $\lambda^c_k(w)$ for every object class realization, overall maintaining $|W|$ hybrid beliefs in parallel. While theoretically this kind of maintenance is computationally expensive, in reality many class realizations are with probability close to zero, allowing us to prune the beliefs if needed.

In total, $|W|$ hybrid beliefs are maintained to infer $\lambda_{k+1}(w)$ for each. All $\lambda_{k+1}(w)$ together represent $b[\lambda_{k+1}]$ and thus the reward function over it can be computed. 

%--TODO: Connect this to a more general cost function
Another type of cost functions use the continuous belief $\prob{\poses_{k+1}|I_{1:k+1},\his^g_{k+1},D}$. To infer a joint belief from multiple individual hybrid beliefs, we will marginalize by $w$ and $c$ using the following:
%
\begin{equation}
\prob{\poses_{k+1}|I_{1:{k+1}},\his^g_{k+1},D} \approx
\sum_w \sum_c \frac{\lambda^c_{k+1}(w)}{|W|} \cdot b^c_w[\poses_{k+1}].
\end{equation}
%
The resulting expression is a mixture model with a large number of components that might require methods for reducing it, possibly by removing and merging components (see e.g. \VT{[REF]}).
%--------------------------------------------------

Alg.~\ref{alg:PC} summarizes our approach for Multi-Hybrid BSP for the ; For every particle, the corresponding hybrid belief is propagated via the motion model applied on the candidate action. Then, using the propagated belief, we generate measurements. For each $w \in W$, a single $z^g_{k+1}$ and a cloud $\{ \loggamma_{k+1} \}$ with $|W|$ points of $\loggamma_{k+1}$ is generated. \VT{Then, every generated pair $z^g_{k+1}, \{ \loggamma_{k+1} \}$ is used to create an update realization of $b[\lambda_{k}]$ by updating individual $\lambda_{k}$ particles in it with the corresponding predicted $\loggamma_{k+1}$.} If the reward function is $H(\lambda_{k+1})$, we assume a distribution over $\lambda_{k+1}$ for each $b[\lambda_{k+1}]$, and finally the entropy is averaged to get the objective function value. In the next section, we discuss two possible options for the distribution assumed for $b[\lambda_{k+1}]$ and make a comparison between them.

\begin{algorithm}[t]
	\caption{Myopic Multi-Hybrid Belief Space Planning} 
	\label{alg:PC} 
	\flushleft
	
	\begin{algorithmic}[1]
		\Require{Set of hybrid beliefs $\{ hb_w[\poses_k,c] \}_w$, action $a_k$.}
		%-->
		\For{$w \in W$}
		
		\State{$hb_w[\poses_{k+1}^-,c] \gets hb_w[\poses_k,c] \cdot \motionmodel_k$}
		\State{$z^g_{k+1}, \{ \loggamma_{k+1} \} \gets \text{SimulateObs}(hb_w[\poses_{k+1}^-,c])$}
		
		\EndFor
		%<--
		\State{$J \gets 0$}
		
		%-->
		\For{$z^g_{k+1}, \{ \loggamma_{k+1} \} \in \{ z^g_{k+1}, \{ \loggamma_{k+1} \} \}$}
		
		\State{$\{\lambda_{k+1}\} \gets \emptyset$}
		%-->
		\For{$w \in W $}
		
		\State{$hb_w[\poses_{k+1},c] \gets$}\par \hskip\algorithmicindent {$\text{UpdateHB}(hb_w[\poses_{k+1}^-,c], z^g_{k+1}, \loggamma_{k+1})$ }
		
		\State{$\{\lambda_{k+1}\} \gets \{\lambda_{k+1}\} \cup \omega_{w,k}$}
		
		
		%<--
		\EndFor
		
		\State{$b[\lambda_{k+1}] \gets \text{InferDistribution}\left( \{\lambda_{k+1}\} \right)$}
		\State{$r(b[\lambda_{k+1}]) \gets \text{Entropy}(b[\lambda_{k+1}])$}
		
		\State{$J \gets J + r(b[\lambda_{k+1}])$}
		
		%<--
		\EndFor \\
		\Return{$J$}
	\end{algorithmic}
\end{algorithm}

%----------------------------------------------------------------------------------

\subsection{Distribution of $b[\lambda_{k+1}]$}

Planning over the entropy of $b[\lambda_{k+1}]$ accounts for both classification score ambiguity and epistemic model uncertainty. We require first to infer the distribution parameters, then to compute the entropy. One must consider the dimensionality and expressibility (i.e. how many distributions can be described?) for both of the candidates. Sec.~\ref{sec:Dir_Dist_Lambda} and Sec.~\ref{sec:LG_Dist_Lambda} detail Dirichlet and Logistical Gaussian distributions for $b[\lambda_{k+1}]$ respectively. Sec.~\ref{sec:Dir_LG_discussion} discusses the differences between utilizing both distributions.
To simplify notations, all of the variables in this section are considered at time $k+1$, so we drop the time step index.

%--O--
\subsubsection{Logistic-Gaussian Distribution for $b[\lambda]$}\label{sec:LG_Dist_Lambda}

One option is to assume that $b[\lambda]$ is Logistic Gaussian (LG) distributed. This distribution (with PDF as in Eq.~\eqref{eq:Logistical_Gaussian_PDF}) is a representation of distribution over probability vectors in which samples necessarily satisfy all the condition of probability vectors, presented in Sec.~\ref{sec:Gamma_Lambda} for $\gamma$. While this distribution doesn't have analytical expression for expectation and covariance, it isn't required for planning. 

We can infer the parameters of $b[\lambda]$ by applying the logit transformation from Eq.~\eqref{eq:Logit_transformation} for each $\lambda(w)$ to get $\loglambda(w)$. Then, the Logistical Gaussian parameters can be inferred as Gaussian expectation and covariance from $\loglambda(w)$ realizations. 

Eventually, when planning over the entropy of $\lambda$, the LG distribution doesn't have a closed form expression for it. As Logistical Gaussian is formed from a variable transformation of the Gaussian distribution, it allows us to write the general form of the entropy for $\lambda$, with the complete derivation can be seen in the appendix \VT{[REF]}: 
%
\begin{equation}\label{eq:Entropy_LG_total}
\begin{split}
H(\lambda) = & H(\loglambda) + \sum_{i=1}^{m-1} \mathbb{E}[\loglambda^i] \\
& - \int_{\loglambda} \log \left( 1 + \sum_{i=1}^{m-1} e^{\loglambda^i} \right) \mathcal{N} d\loglambda,
\end{split}
\end{equation}
%
where $\mathcal{N}$ is the PDF of $\loglambda$ which is Gaussian distributed with expectation $\mathbb{E}[\loglambda]$ and covariance $Cov(\loglambda)$. As $\loglambda$ is Gaussian, $H(\loglambda) = 0.5 \cdot \log (2\pi e |Cov(\loglambda)|)$. The integral in Eq.~\eqref{eq:Entropy_LG_total} to the best of our knowledge doesn't have an analytical solution, thus the entropy must be either estimated numerically, or via bounds. An upper bound (full derivation in Appendix \VT{[REF]}) can be computed as follows:
%
\begin{equation}\label{eq:LG_entropy_upper_bound}
H(\lambda) \leq H(\loglambda) + \sum_{i=1}^{m-1} \mathbb{E}(\loggamma^i) - m \cdot \max_i \{ 0 , \mathbb{E}(\loggamma^i) \},
\end{equation}
%
and similarly a lower bound:
%
\begin{equation}\label{eq:LG_entropy_lower_bound}
\begin{split}
H(\lambda) \geq & H(\loglambda) + \sum_{i=1}^{m-1} \mathbb{E}(\loggamma^i) \\ & - m \cdot \max_i \{ 0 , \mathbb{E}(\loggamma^i) \} - m \log m.
\end{split}
\end{equation}
%
One can observe from this upper bound that $H(\loglambda)$ is necessarily larger than $H(\lambda)$ as $\loggamma$ isn't subjected to the probability vector constraints, thus $\mathbb{E}(\loggamma^i)$ can be negative for every $i$ and $\sum_{i=1}^{m-1} \mathbb{E}(\loggamma^i) - m \cdot \max_i \{ 0 , \mathbb{E}(\loggamma^i) \}$ is necessarily non-positive.

Fig.~\ref{fig:LG_Entropy} presents the entropy values of $b[\lambda]$ in the case of two candidate classes. As it has a single degree of freedom, two parameters can fully describe the distribution. The figure shows that the farther $\mathbb{E}[\loglambda]$ is from zero, i.e. the closer $\mathbb{E}[\lambda^1]$ to either one or zero, the smaller the entropy gets in general. The effect is more pronounced in the case where $Var(\loglambda)$ is small. If we aim to minimize the entropy during planning, the robot will aim to reach regions where $\mathbb{E}[\lambda]$ is close to the edges of the simplex, and have smaller posterior epistemic uncertainty.

\begin{figure}[!htbp]
	
	\includegraphics[width=\textwidth]{LG_entropy.eps}
	\caption{Entropy of a one dimensional Logistical Gaussian that corresponds to two dimensional probability vector $\gamma$. The $x$ and $y$ axis represent $\mathbb{E}(\loggamma)$ and $Var(\loggamma)$ respectively. Blue to yellow colors correspond to low to high entropy.}
	
	\label{fig:LG_Entropy}
\end{figure}

\subsubsection{Dirichlet Distribution for $b[\lambda]$}\label{sec:Dir_Dist_Lambda}

The other option assumes $b[\lambda]$ is Dirichlet distributed. This distribution is a natural representation of distribution over probability vectors in which samples necessarily satisfy all the conditions of probability vectors presented in Sec.~\ref{sec:Gamma_Lambda}.

The Dirichlet distribution is parametrized by a parameter set $\alpha \doteq \{ \alpha_1,...,\alpha_m \}$, and the PDF is:
%
\begin{equation}
Dir(\lambda;\alpha) = \frac{1}{B(\alpha)} \prod_{i=1}^m (\lambda^i)^{\alpha_i - 1},
\end{equation}
%
with $\lambda^i$ being the $i$'th class probability, and $B(\alpha)$ a normalization constant that is defined as follows:
%
\begin{equation}
B(\alpha) \doteq \frac{\prod_{i=1}^m \Gamma(\alpha_i)}{\Gamma\left( \sum\alpha \right)},
\end{equation}
%
where $\Gamma(\cdot)$ is the Gamma function and $\sum\alpha \doteq \sum_{i=1}^m \alpha_i$ for shorthand.
The distribution's expectation, that describe the posterior classification results, is:
%
\begin{equation}
\mathbb{E}(\lambda^i) = \frac{\alpha_i}{\sum \alpha},
\end{equation}
%
the covariance, that describe the uncertainty, is:
%
\begin{equation}
Cov(\lambda^i, \lambda^j) = \begin{cases}
\frac{\mathbb{E}(\lambda^i) (1 - \mathbb{E}(\lambda^i))}{\sum\alpha + 1}, & i = j \\
\frac{\mathbb{E}(\lambda^i) \mathbb{E}(\lambda^j)}{\sum\alpha + 1}, & i \neq j.
\end{cases}
\end{equation}
%
From the above expression from expectation and covariance we can infer that the ratios between the parameters determine the expectation, and the sum of all the parameters determines the covariance, or uncertainty. Eventually, informative distribution of $\lambda$ will have a single parameter that has significantly higher value than the rest, and a larger sum in parameter value if the ratio is not large. How informative this distribution is can be described by Dirichlet distribution's entropy:
%
\begin{equation}\label{eq:Dir_Entropy}
H(\lambda) \doteq \log B(a) + (\sum\alpha - m) \psi(\sum\alpha) - \sum_{i=1}^m (\alpha_i - 1) \psi(\alpha_i),
\end{equation}
%
where $\psi(\cdot)$ is the digamma function. This entropy takes the maximal value when $\alpha_i = 1,\; \forall i$, and at the "edges" of the distribution, where a single parameter is much larger than the others, the entropy is the lowest. If one of the parameters is zero, then $H(\lambda) = -\infty$, as $\psi(0) = -\infty$. This behavior of the entropy can be observed in Fig.~\ref{fig:2D_Entropy_Graph} that shoes an example of a two dimensional distribution. Eventually, as seen farther into the paper, we use the Dirichlet entropy as a cost function which doesn't require hyper-parameter tuning (unlike in \cite{Lutjens18arxiv}).

The Dirichlet parameters $\alpha$, given a cloud of probability vectors $\{\lambda_k\}$, can be estimated in an iterative manner as follows:
%
\begin{equation}
\psi(\alpha_i^{\text{new}}) = \psi(\sum_{j=1}^m \alpha_j^{old}) + \log \bar{\lambda}_k^i,
\end{equation}
%
where $\bar{\lambda}^i$ is the average of all $\lambda^i$ for class $i$ in $\{\lambda\}$.

\begin{figure}[!htbp]
	
	\includegraphics[width=\textwidth]{Dir_Entropy.png}
	\caption{Entropy of a two dimensional Dirichlet distribution as a function of log of parameters. Blue to yellow colors correspond to low to high entropy values.}
	
	\label{fig:2D_Entropy_Graph}
\end{figure}

%--O--
\subsubsection{Comparison Between Dirichlet and Logistical-Gaussian}\label{sec:Dir_LG_discussion}

While the parameter inference for Dirichlet distribution requires a numeric computation and involves digamma functions that require numeric computation by themselves, the Logistical Gaussian distribution uses the known Gaussian parameter estimation after transforming the data-points to logit space. This allows for  more accurate inference for Logistical Gaussian parameters. Because of the larger number of parameters for Logistical Gaussian, this distribution is more expressive than the Dirichlet distribution, but the parameter inference is slower for larger number of candidate classes.

Another point of comparison is the computation of the entropy. The entropy of Dirichlet distributed variables has an analytical form that contains Gamma functions that must be computed numerically. However, this computation is fast and accurate. On the other hand, the Logistical Gaussian distribution doesn't have an analytical form and must be approximated either directly from the data-points, or requires using bounds. In addition, the computation requires a determinant operation over $m \times m$ size matrices, which can get computationally expensive for a large $m$ (e.g. ImageNet-trained \cite{Deng2009cvpr} classifiers with 1000 candidate classes). Approximation directly from data will require inverting the covariance matrix as well, which is by itself poses significant computational cost. The upper bound in Eq.~\eqref{eq:LG_entropy_upper_bound} carries the same computational effort as computing the Dirichlet entropy for the same number of classes.

For small number of samples for probability vectors (i.e. a small number of parallel hybrid beliefs in our case as we will see in Sec.~\ref{sec:approach}), Logistical Gaussian distribution risks its covariance matrix getting singular, while the Dirichlet distribution can handle a small number of samples, even as low as two. That gives a major advantage to the Dirichlet distribution in that regard.

Fig.~\ref{fig:Dir_LG_comp} presents a comparison between the two distribution in terms of computational effort and value of the entropy. In all figures, the x-axis is number of candidate classes, and for each a dataset of 1000 class probability vectors was sampled. Fig.~\ref{fig:Fig_time_inf} the inference time was measured, clearly showing an advantage for Dirichlet distribution for high dimensional probability vectors despite the inference process for Dirichlet distribution containing functions that must be numerically computed. Fig.~\ref{fig:Fig_time_ent} presents the computational time for entropy computation, both for the bounds and the numerical estimation. Here the Dirichlet distribution holds a significant advantage against numerical computation of the entropy. Fig.~\ref{fig:Val_fig_ent} presents the entropy values for Dirichlet, numerical LG, lower and upper bounds. In general the upper bound tend to be close to the numerical solution for fewer candidate classes. in addition, the entropy for Dirichlet distribution tends to be higher. Finally Fig.~\ref{fig:Log_likelihood_graph} presents the average log-likelihood values for Dirichlet distribution and LG, where LG shows an advantage because of its higher expressivity (i.e. larger amount of parameters).

In conclusion, One may ask: which distribution should be used? The tradeoff is between distribution expressiveness and computational effort. While Logistical Gaussian is more expressive because of a larger number of parameters, the computation effort is significantly larger than for Dirichlet distribution for larger $m$'s. Also, Dirichlet distribution, unlike the Logistical Gaussian can manage a very small number of probability vector samples. 

\begin{figure*}[!htbp]
	
	\begin{subfigure}[b]{0.23\textwidth}
		\includegraphics[width=\textwidth]{Fig_time_inf.eps}
		\caption{Inference time}\label{fig:Fig_time_inf}
	\end{subfigure}
	%
	\begin{subfigure}[b]{0.23\textwidth}
		\includegraphics[width=\textwidth]{Fig_time_ent.eps}
		\caption{Entropy time}\label{fig:Fig_time_ent}
	\end{subfigure}
	%
	\begin{subfigure}[b]{0.23\textwidth}
		\includegraphics[width=\textwidth]{Val_fig_ent.eps}
		\caption{Entropy value}\label{fig:Val_fig_ent}
	\end{subfigure}
	%
	\begin{subfigure}[b]{0.23\textwidth}
		\includegraphics[width=\textwidth]{Log_likelihood_graph.eps}
		\caption{Entropy value}\label{fig:Log_likelihood_graph}
	\end{subfigure}
	
	\caption{This figure presents a comparison between Dirichlet and Logistical Gaussian (denoted LG) in terms of computational time, entropy, and log-likelihood values. \textbf{(a)} presents a computational time comparison between Dirichlet and LG for inference as a function of probability vector dimension. Similarly \textbf{(b)} presents a computational time for entropy computation, both for numerical and upper bound. \textbf{(c)} presents a value comparison between the different entropy computations. \textbf{(d)} presents a comparison for average log-likelihood between values given the number of candidate classes.}
	\label{fig:Dir_LG_comp}
\end{figure*}

%----------------------------------------------------
\subsection{Computational Complexity}

With $m$ candidate classes, and $n$ objects, the number of possible class realizations per particle is $m^n$. For traditional SLAM using iSAM2, the time computational complexity for inferring the parameters for $\prob{\poses_k|C,\loggamma_{1:k},\his^g_k}$ is $O(k^{1.5})$, and at worst $O(k^3)$ for loop closures \cite{Kaess12ijrr}. To compute an individual $\lambda_k$ particle, we must account for the attached $\prob{\poses_k|C,\loggamma_{1:k},\his^g_k}$, and thus the time computational effort at worst is $O(m^n k^3)$. Eventually we maintain $|W|$ particles, and therefore the overall time computational complexity for $b[\lambda_k]$ inference is $O(|W|m^n k^3)$ at worst. For planning, we have to take into account that we sample $|W|$ pairs of $z^g_{k+1}$ and $\{ \gamma_{k+1} \}$, therefore for each pair we must compute a separate $b[\lambda_{k+1}]$. That amounts to the worst case complexity of $O(|W|^2 m^n k^3)$.

In reality, the $O(k^3)$ worst case time complexity is only present in loop closures, and most of the time the complexity is $O(k^{1.5})$. The computational complexity can be further reduced by pruning low probability classes for individual particles, but this can induce a problem where certain realization gets "locked" in either probability 0 or 1, rendering the possibility of probability changing for the said realization impossible. 

For memory complexity, we require the latest robot pose, and the $n$ poses \& $m$ sized class probability vector for every object per $\lambda$ particle. All in all, we must maintain $O(n m^n)$ random variables in memory per particle, and $O(|W| n m^n)$ variables for $b[\lambda]$. This also can be reduced by pruning the low probability class realizations.

%---------------------------------------------------------------------
\subsection{Joint Pose and $\lambda$ Inference Via Factor Graph Optimization}

In this subsection we present an alternative approach for inference which maintains the joint belief of $\poses_k$ and $\lambda_k$, that under certain conditions, that we will detail farther down in this section, can be significantly more computationally efficient than the Multi-Hybrid approach. First, we define the aforementioned joint belief:
%
\begin{equation}
	b[\loglambda_k,\poses_k] \doteq \prob{\loglambda_k,\poses_k|I_{1:k},\his^g_k,D}.
\end{equation}
%
To update this belief recursively, we must express it as a function of the prior $b[\loglambda_{k-1},\poses_{k-1}]$; To do so, we marginalize by $\loglambda_{k-1}$:
%
\begin{equation}\label{eq:Lambda_X_inference}
	b[\loglambda_k,\poses_k] = \int_{\loglambda_{k-1}} \prob{\loglambda_{k-1:k},\poses_k|I_{1:k},\his^g_k,D}
	d \loglambda_{k-1},
\end{equation}
%
and using the Bayes rule we can derive an expression to recursively update $b[\loglambda_k,\poses_k]$:
%
\begin{equation}
\begin{split}
	b[\loglambda_k,\poses_k] = & \eta \int_{\loglambda_{k-1}} 
	\prob{\loglambda_k|\loglambda_{k-1},I_k,D,x_k^{rel}} \cdot
	\motionmodel_k \cdot \\ & \cdot
	\prob{z^g_k|x_k^{rel}} \cdot
	b[\loglambda_{k-1},\poses_{k-1}] d\loglambda_{k-1}.
\end{split}
\end{equation}
%
The novel term in the above equation is $\prob{\loglambda_k|\loglambda_{k-1},I_k,D,x_k^{rel}}$; We denote this as the $\loglambda_k$ propagation model. The output cloud $\{\gamma_k\}$ is a function of the image and by extension $\{\loggamma_k\}$, the classifier and its training set, thus the propagation model can be written as $\prob{\loglambda_k|\loglambda_{k-1},\{\loggamma_k\},x_k^{rel}}$. The reasoning behind this model is the following update using Bayes rule for $\lambda_k^c$ given $\lambda_{k-1}^c$ and $\loggamma_k$ for class $c$ given $x^{rel}_k$:
%
\begin{equation}
	\lambda_k^c = \eta \cdot \lambda_{k-1}^c \cdot \prob{\loggamma_k|c,x^{rel}_k},
\end{equation}
%
where $\eta$ is a normalizing constant equal for all $c$. When $\lambda_k$ is cast into logit space, the above equation transforms into the following sum, written in a vector form:
%
\begin{equation}
	\loglambda_k = \loglambda_{k-1} + l\mathcal{L}^s_k,
\end{equation}
%
where $l\mathcal{L}^s_k$ is defined as:
%
\begin{equation}
\begin{split}
	l\mathcal{L}^s_k \doteq & \bigg[ \log \left( \frac{\prob{\loggamma_k | c=1,x^{rel}_k}}
	{\prob{\loggamma_k | c=m,x^{rel}_k}} \right) , ... , \\
	& \log \left( \frac{\prob{\loggamma_k | c=m-1,x^{rel}_k}}
	{\prob{\loggamma_k | c=m,x^{rel}_k}} \right) \bigg]^T.
\end{split}
\end{equation}

Let us describe the condition for which $b[\loggamma_k,\poses_{k}]$ is accurately represented in this section, presented in the following Lemma:
%
\begin{lemma}\label{lemma:FGCondition}
	For Gaussian distributed $\loggamma_k$ and Gaussian distributed classifier uncertainty models $\prob{\loggamma_k|c,x^{rel}_k}$ with covariance matrix $\Sigma_c$, if the Covariance matrices for the models are identical, i.e. $\Sigma_{c=i} \equiv \Sigma_{c=j}$ given $x^{rel}_k$, then $l\mathcal{L}^s_k$ is Gaussian distributed.
\end{lemma}

\begin{proof}
	We will prove  by construction, with writing the PDF of the classifier uncertainty model for the $i$'th element of $l\mathcal{L}^s_k$. The model for class $i$ has an expectation $h_{c=i}$ and a covariance matrix $\Sigma_{c=i}$;  We can write the following:
	%
	\begin{equation}\label{eq:Condition_Develop_1}
	\begin{split}
		l\mathcal{L}^s_{k,i} & = \log \left( \frac{(2\pi)^{\frac{m-1}{2}} \sqrt{|\Sigma_{c=m}}|
		e^{ -\frac{1}{2}||\loggamma - h_{c=i} ||^2_{\Sigma_{c=i}}}}
		{(2\pi)^{\frac{m-1}{2}} \sqrt{|\Sigma_{c=i}}|
		e^{ -\frac{1}{2}||\loggamma - h_{c=m} ||^2_{\Sigma_{c=m}}}} \right) \\ 
		& = - \frac{1}{2} \log(|\Sigma_{c=i}|) + \frac{1}{2} \log(|\Sigma_{c=m}|) \\
		& -\frac{1}{2}||\loggamma - h_{c=i} ||^2_{\Sigma_{c=i}} +\frac{1}{2}||\loggamma - h_{c=m} ||^2_{\Sigma_{c=m}}.
	\end{split}
	\end{equation}
	%
	Now, applying the condition $\Sigma_{c=i} \equiv \Sigma_{c=j}$, and denoting both as $\Sigma_c$ we get the following expression:
	%
	\begin{equation}
	\begin{split}
		l\mathcal{L}^s_{k,i} = & \loggamma_k^T \Sigma_{c}^{-1} h_{c=i} -
		\frac{1}{2} h_{c=i}^T \Sigma_{c}^{-1} h_{c=i} \\ & -
		\loggamma_k^T \Sigma_{c}^{-1} h_{c=m} +
		\frac{1}{2} h_{c=m}^T \Sigma_{c}^{-1} h_{c=m}.
	\end{split}
	\end{equation}
	%
	From the above equation, if $\loggamma_k$ is a multi-variate Gaussian random variable, then $l\mathcal{L}^s_{k,i}$ is a linear combination of Gaussian random variables, therefore Gaussian by itself. This scheme can be extended for every $i = 1,...,m-1$.
\end{proof}

In general, the classifier model covariances won't be equal; Therefore, Eq.~\ref{eq:Condition_Develop_1} will include a quadratic expression of $\loggamma_k$, making $l\mathcal{L}^s_{k,i}$ a mixture of Gaussian and Generalized Chi distributions, effectively introducing additional modals that potentially grow in number with future time steps. To combat this, the models' covariances must be "close" to each other to approximately describe $l\mathcal{L}^s_{k,i}$ as a Gaussian.

If $l\mathcal{L}^s_k$ is assumed Gaussian via moment matching or other methods, it will only approximate the true distribution of $l\mathcal{L}^s_k$ with the accuracy dependent on the "distance" between it's covariance matrices given $x^{rel}_k$. This distance can be represented by, for example, Forbenius Norm. \VT{This distance metric is used in the paper, and is defined for given information matrices $\Sigma^{-1}_{c=i}$ and $\Sigma^{-1}_{c=m}$ as:
%
\begin{equation}
	f_{\Sigma^{-1}_{c=i},\Sigma^{-1}_{c=m}} = Tr \left( (\Sigma^{-1}_{c=i} - \Sigma^{-1}_{c=m}) \cdot
	(\Sigma^{-1}_{c=i} - \Sigma^{-1}_{c=m})^T \right).
\end{equation}
%
The Forbenius norm can be inserted into the classifier uncertainty models' loss function for training, enforcing sufficiently close covariances between different models such that the approach presented in this section can be used.}

Assuming the conditions for Lemma \ref{lemma:FGCondition} are true or approximately true, we can integrate the model $\prob{\loglambda_k|\loglambda_{k-1},I_k,x_k^{rel}}$ from Eq.~\eqref{eq:Lambda_X_inference} within SLAM framework as a non-linear factor as follows:
%
\begin{equation}\label{eq:logit_l_exp_1}
	\prob{\loglambda_k|\loglambda_{k-1},I_k,x_k^{rel}} = 
	\mathcal{N}\left(\loglambda_{k-1} + \mathbb{E}[l\mathcal{L}^s_k],Cov(l\mathcal{L}^s_k)\right).
\end{equation}

The term $l\mathcal{L}^s_k$ is dependent on $\loggamma_k$, $x_k^{rel}$, and the all the classifier models. If we get from the classifier a cloud $\{ \gamma_k \}$, each $\gamma_k \in \{ \gamma_k \}$ can be transformed using the logit transformation to $\loggamma_k$, and from $\{ \loggamma_k \}$ we can infer a maximum likelihood estimation for expectation vector $\mathbb{E}(\loggamma_k)$ and covariance matrix $\Sigma(\loggamma_k)$. Using Eq.~\eqref{eq:logit_l_exp_1} we can describe $l\mathcal{L}^s_k$ as follows:
%
\begin{equation}
	l\mathcal{L}^s_k = \Phi_1 \loggamma_k - \frac{1}{2} \Phi_2
\end{equation} 
%
where the matrix $\Phi_1 \in \mathbb{R}^{(m-1) \times (m-1)}$ and the vector $\Phi_2 \in \mathbb{R}^{m-1}$ depend on the individual classifier models and $x_k^{rel}$. Using Eq.~\eqref{eq:logit_l_exp_1}, the term $\Phi_1$ is defined as:
%
\begin{equation}
	\Phi_1 \doteq \left[ 
	\begin{array}{c}
	h^T_{c=1} \Sigma^{-1}_{c=1} - h^T_{c=m} \Sigma^{-1}_{c=m} \\
	\vdots \\
	h^T_{c=m-1} \Sigma^{-1}_{c=m-1} - h^T_{c=m} \Sigma^{-1}_{c=m}
	\end{array}
	\right]
\end{equation}
%
and $\Phi_2$ is defined as:
%
\begin{equation}
	\Phi_2 \doteq \left[
	\begin{array}{c}
	h^T_{c=1} \Sigma^{-1}_{c=1} h_{c=1} - h^T_{c=m} \Sigma^{-1}_{c=m} h_{c=m} \\
	\vdots \\
	h^T_{c=m-1} \Sigma^{-1}_{c=m-1} h_{c=m-1} - h^T_{c=m} \Sigma^{-1}_{c=m} h_{c=m}
	\end{array}
	\right].
\end{equation}

If $\Phi_1$ isn't a singular matrix, and given $x_k^{rel}$, the novel factor can be written as:
%
\begin{equation}\label{eq:JLP_Factor}
\begin{array}{c}
	\prob{\loglambda_k|\loglambda_{k-1},I_k,D,x_k^{rel}} = \\
	\mathcal{N} \left( \loglambda_{k-1} + \Phi_1 \mathbb{E}(\loggamma_k) - \frac{1}{2} \Phi_2,
	\Phi_1 \Sigma(\loggamma_k) \Phi_1^T \right).
\end{array}
\end{equation}
%
The term $\Phi_1 \Sigma(\loggamma_k) \Phi_1^T$ is positive definite when $\Phi_1$ isn't singular, but in practice we can't guarantee this condition. If there is some $x^{rel}_k$ for classes $c=i$ and $c=j$ where $h_{c=i} = h_{c=j}$ and $\Sigma_{c=i} = \Sigma_{c=j}$, then at that point $\Phi_1$ is singular. This means: at that certain $x^{rel}_k$, we can't differentiate between the two classes with the given classifier models. To keep $\Phi_1 \Sigma(\loggamma_k) \Phi_1^T$, we add to it an identity matrix multiplied by a small positive constant $\epsilon \cdot I^{(m-1) \times (m-1)}$. The factor Eq.~\eqref{eq:JLP_Factor} is a four variable factor that can be inserted into a graph structure that can be optimized using standard SLAM methods. To this end, the marginal posterior $b[\loglambda_k]$ uncertainty takes into account the uncertainty of $b[\loglambda_{k-1}]$, current pose uncertainty, and the uncertainty from $\prob
{\loggamma_k|I_k,D}$. 

The advantage of this approach compared to Multi-Hybrid is that it doesn't require maintaining multiple hybrid beliefs. It maintains a single continuous belief that encompasses all poses and object classes while reasoning about classifier epistemic uncertainty, allowing a rich, viewpoint dependent representation of object class probabilities. The disadvantage of this approach is forcing $\loglambda$ to be LG distributed, which scales poorly with a high number of candidate classes and its entropy lacks a closed form expression. In addition, this approach doesn't provide accurate inference when general classifier models are used, i.e. it's covariance matrices aren't forced to be close to each other.

\subsection{Joint Pose and $\lambda$ planning}

Similarly to the Multi-Hybrid approach, we must reason about the generation of new measurements. In the JLP approach, we need to provide the inference algorithm the parameters of the LG distribution of predicted $\gamma_{k+1}$ instead a set of samples; These parameters can be drawn directly from the appropriate classifier uncertainty model given class $c$ and relative pose $x_k^{rel}$. The following generative model shows the process of creating new measurements for the JLP approach:
%
\begin{equation}\label{eq:Gen_Model_JLP}
\begin{array}{c}
	\mathbb{E}(\loggamma_{k+1}), \Sigma(\loggamma_{k+1}) = f \left( c , x^{rel}_{k+1} \right) \\
	z^G_{k+1} \sim \prob{z^G_k|x^{rel}_{k+1}} \\
	c \sim Cat(\lambda_k) \\
	\lambda_k, x^{rel}_{k+1} \sim \motionmodel_{k+1} \cdot b[\loglambda_k,\poses_k] ,
\end{array}
\end{equation}
%
A note on sampling the maximum likelihood of the states: while taking the maximum likelihood estimation as a single sample is possible, an issue arises where the algorithm plans only according to the classifier uncertainty model of the most likely class, whether it is the ground truth class or not.




%----------------------------------------------------
%\subsection{Passive Inference}
%
%Eventually, the robot will perform an action and will potentially get raw measurements, and we must reason about incorporating these measurements and update a belief that represents all states of the robot and environment. The important states to consider are robot and object poses $\poses_k$, and the object's posterior class probability $\lambda_k$, culminating in the following belief given raw images $I_{1:k}$, geometric measurement history $\his^g_k$, and classifier training set $D$. As $\lambda_k$ is bounded and thus can't be described by a Gaussian, we use the logit transformation for $\lambda_k$ and describe the belief using $\loglambda_k$:
%%
%\begin{equation}
%	b[\loglambda_k,\poses_k] \doteq \prob{\loglambda_k,\poses_k|I_{1:k},\his^g_k,D}.
%\end{equation}
%%
%To update this belief recursively, we must express it as a function of the prior $b[\loglambda_{k-1},\poses_{k-1}]$; To do so, we marginalize by $\loglambda_{k-1}$:
%%
%\begin{equation}
%	b[\loglambda_k,\poses_k] = \int_{\loglambda_{k-1}} \prob{\loglambda_{k-1:k},\poses_k|I_{1:k},\his^g_k,D}
%	d \loglambda_{k-1},
%\end{equation}
%%
%and using the Bayes rule we can derive an expression to recursively update $b[\loglambda_k,\poses_k]$:
%%
%\begin{equation}
%\begin{split}
%	b[\loglambda_k,\poses_k] = & \eta \int_{\loglambda_{k-1}} 
%	\prob{\loglambda_k|\loglambda_{k-1},I_k,D,x_k^{rel}} \cdot
%	\motionmodel_k \cdot \\ & \cdot
%	\prob{z^g_k|x_k^{rel}} \cdot
%	b[\loglambda_{k-1},\poses_{k-1}] d\loglambda_{k-1}.
%\end{split}
%\end{equation}
%%
%The novel term in the above equation is $\prob{\loglambda_k|\loglambda_{k-1},I_k,D,x_k^{rel}}$; We denote this as the $\loglambda_k$ propagation model. The output cloud $\{\gamma_k\}$ is a function of the image and by extension $\{\loggamma_k\}$, the classifier and its training set, thus the propagation model can be written as $\prob{\loglambda_k|\loglambda_{k-1},\{\loggamma_k\},x_k^{rel}}$. The reasoning behind this model is the following update using Bayes rule for $\lambda_k^c$ given $\lambda_{k-1}^c$ and $\loggamma_k$ for class $c$ given $x^{rel}_k$:
%%
%\begin{equation}
%	\lambda_k^c = \eta \cdot \lambda_{k-1}^c \cdot \prob{\loggamma_k|c,x^{rel}_k},
%\end{equation}
%%
%where $\eta$ is a normalizing constant equal for all $c$. When $\lambda_k$ is cast into logit space, the above equation transforms into the following sum, written in a vector form:
%%
%\begin{equation}
%	\loglambda_k = \loglambda_{k-1} + l\mathcal{L}^s_k,
%\end{equation}
%%
%where $l\mathcal{L}^s_k$ is defined as:
%%
%\begin{equation}
%\begin{split}
%	l\mathcal{L}^s_k \doteq & \bigg[ \log \left( \frac{\prob{\loggamma_k | c=1,x^{rel}_k}}
%	{\prob{\loggamma_k | c=m,x^{rel}_k}} \right) , ... , \\
%	& \log \left( \frac{\prob{\loggamma_k | c=m-1,x^{rel}_k}}
%	{\prob{\loggamma_k | c=m,x^{rel}_k}} \right) \bigg]^T.
%\end{split}
%\end{equation}
%
%If $\loglambda_k$ is Gaussian (i.e. $\lambda_k$ is LG distributed), we can integrate this propagation model within SLAM framework as a non-linear factor as follows:
%%
%\begin{equation}
%	\prob{\loglambda_k|\loglambda_{k-1},\{\loggamma_k\},x_k^{rel}} = 
%	\mathcal{N}\left(\loglambda_{k-1} + \mathbb{E}[l\mathcal{L}^s_k],Cov(l\mathcal{L}^s_k)\right).
%\end{equation}
%
%The term $l\mathcal{L}^s_k$ is dependent on $\loggamma_k$, $x_k^{rel}$, and the all the classifier models.
%It is a random variable because $\loggamma_k$ is a random variable. To the best of our knowledge, there is no analytical expression for $\mathbb{E}[l\mathcal{L}^s_k]$ and $Cov(l\mathcal{L}^s_k)$ as a function of parameters of $\prob{\loggamma_|I_k,D}$, therefore these terms must be computed numerically from $l\mathcal{L}^s_k$ particles.
%
%%
%%----------------------------------------------------
%


%-----------------------------------
%----------------------------------

\section{Epistemic Uncertainty Aware BSP: Multiple Objects}

In this section we transition into the more realistic setting of multiple objects within the environment. This transition requires additional definitions, and we will discuss both the Multi-Hybrid approach and the \VT{Joint Factor Graph approach.}

\subsection{Preliminaries}

Expanding the approach for multiple objects will require new and revised definitions. First, we will define a joint $\Gamma_k$ realization for all objects observed at time $k$ as $\Gamma_k \doteq \{ \gamma_{k,o} \}_{o \in O_{k}}$, where $O_k \in O$ represents the set of all objects observed at time $k$, and $O$ represents the set of all objects in the environment. The classifier comes with a segmentation algorithm that separates the objects observed into sub-images, and for each the classifier outputs a cloud $\{ \gamma_{k,o} \}$, thus we can define a set of clouds observed at time $k$ as $\{ \Gamma_k \} \doteq \{\{ \gamma_{k,o} (w) \}_{w \in W} \}_{o \in O_{k}}$. This set serves us as the semantic measurements history when combining with previous measurements $\his^s_k \doteq \{\Gamma_{1:k} \}$, note that $\Gamma_k$ can be transformed into the logit form $\logGamma_k$. Similarly, we define the set of geometric measurements observed from objects at time $k$ as $Z^g_k \doteq \{z^g_{k,o}\}_{o \in O_k}$, and this serves us as the geometric measurement history when combined with previous measurements $\his^g_k \doteq Z^g_{1:k}$. Finally, the total history includes actions, semantic and geometric measurements $\his_k \doteq \{ \his^g_k, \his^s_k, a_{0:k-1} \}$. 

We define an object class realization as $C \doteq \{(c)_o\}_{o \in O}$. Realization $C$ is a discrete random variable that categorically distributed with $m^n$ elements in it, with each element corresponds to a class hypothesis of all known objects simultaneously. In addition, we include all known object poses within $\poses_k$ as well.

We define the joint posterior class probability vector as:
%
\begin{equation}
	\Lambda_k \doteq \prob{C|\logGamma_{1:k},\his^g_k}
\end{equation}
%
and subsequently the belief over $\Lambda_k$ is:
%
\begin{equation}
	b[\Lambda_k] \doteq \prob{\Lambda_k|I_{1:k},\his^g_k,D}.
\end{equation}
%
As $\Lambda_k$ is a probability vector, rewards over a single object $\lambda_k$ still apply, but the dimension is $m^n$.

%-------------------------------------
\subsection{Multi-Hybrid BSP}

For every $w \in W$, updating $\Lambda_k$ is largely similar to updating $\lambda_k$ in Sec.~\ref{sec:MH_single_lambda_inf} except for few differences. The likelihood terms include all objects $O_k$ observed at time $k$, and the conditional probability over the poses is conditioned on class realization $C$ instead of the class of a single object.
%
\begin{equation}
	\Lambda^C_{k+1} \propto \Lambda^C_k \int_{x^{inv}_{k+1}} \mathcal{L}_{k+1} \cdot \motionmodel_{k+1}  \cdot
	b^C_w[\poses^{inv-}_{k+1}] dx^{inv}_{k+1},
\end{equation}
%
where $\Lambda^C$ denote the posterior probability of class realization $C$, and $x^{inv}_{k+1}$ represents the last robot pose and all poses of objects observed at time $k+1$, i.e. $\poses^{inv}_{k+1} \doteq x_{k+1} \cup \{ x^o \}_{o \in o_{k+1}}$. Likelihood $\mathcal{L}_{k+1}$ now encompasses all the measurement likelihoods of all objects as follows:
%
\begin{equation}
	\mathcal{L}_{k+1} \doteq \prod_{o \in O_{k+1,o}} \prob{\loggamma_{k+1,o}|C,x^o,x_{k+1}} \cdot 
	\prob{z^g_{k+1}|x^o,x_{k+1}}.
\end{equation}
%
The belief $b^C_w[\poses^{inv-}_{k+1}]$ is the propagated belief conditioned on $C$, and marginalized over the uninvolved variables such that $\poses_{k+1} = \poses^{inv}_{k+1} \cup \poses^{\neg inv}_{k+1}$:
%
\begin{equation}
	b^C_w[\poses^{inv-}_{k+1}] = \int_{\poses^{\neg inv}_{k+1}} b_w^C[\poses_k] \cdot \motionmodel_{k+1} d\poses^{\neg inv}_{k+1}.
\end{equation}

The sampling of new measurements works almost identically as in Alg.~\ref{alg:SamplingStrategy}, with the only difference is that we sample a class realization $C$ that encompasses all the objects instead of a class of a single object. The geometric and semantic measurements are sampled on per object basis.

Finally, the cost function for planning over the entropy of $b[\Lambda_{k+1}]$ is identical to the single-object case, except that the dimension of $\Lambda_{k+1}$ is $m^n$, making it advantageous to assume $\Lambda_{k+1}$ is Dirichlet distributed for practical purposes.

%----------------------------------------------------------

\subsection{title}

